Data-Efficient Learning for Complex and Real-Time Physical Problem Solving using Augmented Simulation

Humans quickly solve tasks in novel systems with complex dynamics, without requiring much interaction. While deep reinforcement learning algorithms have achieved tremendous success in many complex tasks, these algorithms need a large number of samples to learn meaningful policies. In this paper, we present a task for navigating a marble to the center of a circular maze. While this system is very intuitive and easy for humans to solve, it can be very difficult and inefficient for standard reinforcement learning algorithms to learn meaningful policies. We present a model that learns to move a marble in the complex environment within minutes of interacting with the real system. Learning consists of initializing a physics engine with parameters estimated using data from the real system. The error in the physics engine is then corrected using Gaussian process regression, which is used to model the residual between real observations and physics engine simulations. The physics engine augmented with the residual model is then used to control the marble in the maze environment using a model-predictive feedback over a receding horizon. To the best of our knowledge, this is the first time that a hybrid model consisting of a full physics engine along with a statistical function approximator has been used to control a complex physical system in real-time using nonlinear model-predictive control (NMPC).

==> material.tex <==
\clearpage
\subsection{All-in-one version}
	\begin{algorithm}
		\caption{Learning procedure}
% 		\label{alg:whole_learning_procedure}
		\begin{algorithmic}[1]
        \State Initialize real system transition buffer $D$
		\While{Termination condition is False}
    		\State Initialize time index $t \leftarrow 0$
    		\State Reset the real system by randomly placing the marble to outermost ring
			\While{Episode termination condition is False}
			    \State Set real state to simulator $\vx^\text{sim}_t \leftarrow \vx^\text{real}_t$
			    \State Compute trajectory $(X^\text{sim}, U^\text{sim})$ using NMPC \label{alg:mpc}
			    \State Apply initial action $\vu_t^\text{real} = \vu_0^\text{sim}$ to the real system
			    \State Store transition $D \leftarrow D \cup \{ \vx_{t}^\text{real}, \vu_{t}^\text{real}, \vx_{t+1}^\text{real}\}$
		        \State Increment time step $t \leftarrow t + 1$
			\EndWhile
			\State \emph{Estimate physical properties} using CMA-ES and $D$ \label{alg:cmaes}
			\State \emph{Train residual GP model} using $D$ \label{alg:residual}
		\EndWhile
		\end{algorithmic}
	\end{algorithm}

\subsection{Separate version}
	\begin{algorithm}
		\caption{Learning procedure}
% 		\label{alg:whole_learning_procedure}
		\begin{algorithmic}[1]
        \State Initialize real-system transition buffer $D$
		\While{Termination condition is False}
		    \State Rollout $N$ episodes and store real transitions into $D$ according to Algorithm.~\ref{alg:rollout}
			\State \emph{Estimate physical properties} using CMA-ES \label{alg:cmaes}
			\State \emph{Train residual GP model} \label{alg:residual}
		\EndWhile
		\end{algorithmic}
	\end{algorithm}

	\begin{algorithm}
		\caption{Rollout an episode using NMPC}
%  		\label{alg:rollout}
		\begin{algorithmic}[1]
		\State Initialize time index $t \leftarrow 0$
		\State Reset the real system by randomly placing the marble to outermost ring
		\While{Episode termination condition is False}
		    \State Set real state to simulator $\vx^\text{sim}_t \leftarrow \vx^\text{real}_t$
    		\State Compute trajectory $(X^\text{sim}, U^\text{sim})$ using NMPC
		    \State Apply initial action $\vu_t^\text{real} = \vu_0^\text{sim}$ to the real system
		    \State Store transition $D \leftarrow D \cup \{ \vx_{t}^\text{real}, \vu_{t}^\text{real}, \vx_{t+1}^\text{real}\}$
	        \State Increment time step $t \leftarrow t + 1$
		\EndWhile
		\end{algorithmic}
	\end{algorithm}



==> rebuttal.tex <==
\newcommand{\review}[1]{{\rm #1}}
\newcommand{\answer}[1]{\textcolor{blue}{#1}}
\newcommand{\assign}[1]{\textcolor{magenta}{#1}}

\section{Author's Response}
We thank the reviewers for their valuable comments and insightful feedback.

To begin with, we agree with many of the reviewers that our claims about the ``human-like'' nature of this model could be softened.
Although our approach for designing the learning agent is inspired by human physical reasoning, it  is not meant to be a model of human cognition.
%people can solve novel manipulation tasks with a handful of trials.
%However, we have toned down the positioning on being human-like and human-level.
To address these concerns, we have changed the title to remove references to ``human-like'' performance, and have reframed both the introduction and discussion to make clear that we are not making claims about whether this model recapitulates cognition, but instead the purpose is to build a sample-efficient, real-time system for physical reasoning. %\assign{Kevin}

We answer the reviewers' questions and comments as follows. Our answers and the corresponding changes in the revised paper are shown in blue.

\subsection{Meta-Review}

\begin{enumerate}
    \item \review{The motivation and positioning on being human-liked and human-level should be toned down. This includes the remarks in the video.} \\
    \answer{We agree that the comparisons to human performance in the original manuscript were too strong and have significantly revised these claims in the current paper -- as mentioned above, we have changed the title, introduction, and discussion to reflect this.} 

    \item \review{Although the authors provided a problem definition section with a list of limitations and assumptions, some important points raised by the reviewers (e.g. related to generality claim of the paper given it is verified in a single task, limitations related to GP, assumptions on distance metric) should be clearly listed/discussed.} \\
    \answer{We would like to answer their points as follows:}
    \begin{enumerate}
        \item \review{generality claim of the paper given it is verified in a single task}\\
        \answer{We agree with this statement, and revised the paper to tone down the generality claim. As seen in the Conclusion section of the paper, we would like to explore this problem in the future work.}

        \item \review{generality claim of assumptions on distance metric: the linear distance to nearest goal that's not feasible for concave paths/obstacles}\\
        \answer{The controller design is based on non-linear trajectory optimization method which is implemented in a recursive fashion and thus, is applicable to wide variety of systems. Please note that quadratic cost function is the most commonly-used cost function in optimal control or trajectory optimization problems. In case of more complex environments, we can use a non-linear programming based trajectory optimization method that allows for more complex constraints and minimum distance constraints in the presence of obstacles. See, for example, the survey on Trajectory optimization~\cite{kelly2017introduction} or our previous work on trajectory optimization~\cite{kolaric2020local} which can incorporate discontinuous constraints. However, we would like to point out that design of cost functions is critical to design of high performance policies (both model-based or model-free RL techniques) and is not a topic covered in this paper. It is, however, a topic of ongoing research.}
        % \item \review{generality claim of assumptions on distance metric: the linear distance to nearest goal that's not feasible for concave paths/obstacles}\\
        % \answer{}
        \item \review{Why did the authors design a lower level controller to move the marble to the next ring? Does it not hurt the generality of the model statement? Did the authors try without such lower level controller?} \\
        \answer{We agree that this simplification does make the controller design a little restrictive. However, this was chosen to account for discontinuity in the state-space of the marble. Designing a trajectory optimization algorithm that can incorporate such discontinuities was out-of-scope for this paper and is left as a future work.}
        \item \review{limitations related to GP: GP aren't feasible for higher-dimensional problems.}\\
        \answer{We agree that GP might have limitations when applied to high dimensional systems. However, we choose this ML model because of the following reasons: many mechanical systems (such as the system considered in this paper) have a low-dimensional physical state, when working with real systems data-efficiency is essential and GP excel in this, non-stationary effects could be in principle modeled using non-stationary kernels, GP is known for its flexibility in describing data corresponding to high prediction accuracy while at the same time providing rigorous variance computation. For these reasons we believe GP was the right choice for the system considered and similar mechanical systems. However, we do not claim that this is the right choice for every system and we reflected this in the text with an additional comment in section IV.B.1). Notice also that the method could use any ML model to learn the residual such as DNN if more appropriate for a specific application. We did not enter in all these details because of space reasoning. }
    \end{enumerate}

    \item \review{The contributions can be clearly stated at the end of the introduction, clarifying the novelties with respect to the existing methods for each contribution.} \\
    \answer{We have summarized the contributions at the end of the introduction.}

    \item \review{Although I believe that such human experiments and comparisons are very valuable, I also believe that the experiments that compare the performance of the model with humans are not well-formed. The experimental design is not fully described as should be in human experiments (who are the subjects, are they naive to the task, do they have previous experience, etc.).}\\
    \answer{We have added detail on our participants at the beginning of section V.C to describe their recruitment and familiarity with the task.} % \assign{Kevin}

    \item \review{The relatively poor performance of the humans might be due to the joystick based control of the platform (rather than physics predictions). The video shows direct control of the platform; how is the performance of the humans in that condition?} \\
    \answer{While we cannot be sure that there is no motor learning beyond the familiarization phase, prior research does suggest that people can quickly adapt to joystick-based motor control \cite{bock2001conditions}. In addition, because there was no statistical evidence for improved times over the five trials, we believe that any additional learning throughout the experiment would be slight, and therefore unlikely to affect the pattern of results that we report. We have included clarifications of this point in section V.C.\\
    All reported human performance (including videos) used joystick control; we did not capture direct control when the maze is held due to the difficulties in localizing the ball when not affixed to the device. The picture with the held maze in the video was for demonstration purposes. We aplogize for the confusion.}
    %, but for clarity we will replace it with the affixed maze.} % \assign{Kevin}

    \item \review{In the results section, "In the middle two rings, ... we can still observe an improvement in the reduction of the variability of the performance": this statement is not supported with data. Additionally, it is difficult to visually see the difference and even if there is slight difference, it is evident that such reduction is not significant. I suggest to remove that statement.}\\
    \answer{Thank you for pointing this out. We agree with you and have removed the corresponding statement.}

    \item \review{It is not clear what is meant by ’the location of the marble is set to the center of each ring’ considering that the forward model should "have the same state that can be observed in the real system"}\\
    \answer{We apologize for the confusion. Please note that this simplification is done in the simulation environment. As described in section III, we simplify the marble dynamics to be independent of the radial dynamics. In the real system, we cannot accurately observe the radial position of the marble (while the marble is in any particular ring) from a vision sensor equipped with our CMS, but we can just figure out which ring the marble is located. For these two reasons, we set the marble to the center location of each ring (and thus ignore any radial dynamics of the marble). We clarified this in section IV-A.}
\end{enumerate}

\subsection{Reviewer2}

\begin{enumerate}
    % \item \review{The paper claims that this method is general but provides no proof.} \\
    % \answer{Please refer to the answer to meta-reviewer 2) a-d).} % \assign{MELCO-MERL}
    \item \review{This work vastly overstates its own importance and contribution and needs to be toned down before I can recommend submission. The paper claims that this method is general but provides no proof (even simulation-to-simulation), the paper sweeps under the rug the fact that many design decisions only work with this kind of problem (e.g. GP aren't feasible for higher-dimensional problems, the linear distance to nearest goal that's not feasible for concave paths/obstacles, the modeling of \_all\_ sim2real differences as a GP, including non-stationary effects), and the framing as "human-level" or "human-like" is slightly inappropriate.} \\
    \answer{We agree that some of the choices made in the proposed algorithm are tailored to the specific system in consideration. As suggested, we toned down the claims on generality in the text of the paper, while the fundamentals of the algorithm are general there are components that need to be engineered (and thus may not be completely automated) for the specific case. For comments on the choice of design decisions and the GP model please refer to the answer to the meta-reviewer 2) b) and d). Please also refer to meta-reviewer 1) for what we have revised related to human-likeness and human-level description.}

    \item \review{Maybe I missed something but the justification for that positioning was "Humans have an intuitive physical understanding and they can learn dynamics on top of that and therefore we take an arbitrary simulator and an arbitrary machine learning model (Gaussian Process model)" (paraphrased from section 5.b). In both the video and the paper, you mention multiple times this being inspired by cognitive science while giving no evidence that the actual underlying process in a human's mind is in any way comparable to what you're doing. And more specifically, if you make vast claims like this, then I expect much more rigor in your experiments: Instead of just having a human baseline on a single task, I'd expect a behavior analysis of how quickly humans adapt to a variety of tasks (not just this one maze) and based on this, I'd expect you to pick from a range of machine learning methods that all serve the same purpose of fine-tuning the simulation. What you presented in the current version of the paper has nothing to do with a "human-like" system other than using an augmented simulator and if that's human-like, then dozens of works that have done the same thing over the last couple of years are also all human-like and therefore this is not a novel feature of your work. If you could remove all references to human-likeness, your paper would be in a much better position. This includes the title which I'd reframe as something like "Solving a maze task via a learning-augmented simulator" (sidenote: the title also currently says "puzzles", plural, and I fail to see a plurality of puzzles).} \\
    \answer{We agree with this statement and have modified the title, introduction, and discussion to better reflect this (as described in our response to the meta-reviewer 1) ).\\
    Also, thank you for your suggestion for changing the title. We have changed the title from "Towards Human-Level Learning of Complex Physical Puzzles" to "Data-Efficient  Learning  for  Complex and Real-Time Physical Problem Solving using Augmented Simulation".} % \assign{Kevin}

    % \item \review{Suggestion to change title}\\
    % \answer{Thank you for your suggestion. We have changed the title from "Towards Human-Level Learning of Complex Physical Puzzles" to "Data-Efficient  Learning  for  Complex,  Real-Time  Physical  Problem Solving  using  Augmented  Simulation".}

    \item \review{I'd recommend the authors add a section to the end of the introduction summarizing their contribution in a bullet point or two and also stating clearly what is NOT in the scope of this work.} \\
    \answer{We have summarized the contributions at the end of the introduction, and have added to the introduction to clarify that modeling human performance is outside the scope of this work.}

    \item \review{The main results are presented only in a plot in Figure 4 and it's entirely unclear if the differences between models per ring are statistically significant. There is also no information on number of trials unless I missed something.}\\
    \answer{Thank you for pointing this out. We have added the number of trials for evaluating the method to the last paragraph of section V-B. We performed 10 experiments for each of the models and for each experiment we measured the time spent in each ring. We have additionally performed statistical analysis to demonstrate that the change in time over trials is statistically significant in the innermost and outermost rings. Please see section V-B.}

    \item \review{The use of weight matrices is very unclear and feels important to the optimization processes (What is Q in eq.8? How did you arrive at 4,4,1,.4 for W in eq.6?)}\\
    \answer{We apologize for the confusion. The W and Q matrices are used to define the weighted norm for the cost function for trajectory optimization and trajectory tracking respectively. These weights represent the coefficient of cost on the four states of the system. The $W$ and $Q$ matrix we use was found empirically (see the original iLQR paper for more details~\cite{tassa2012synthesis}) at the beginning of learning. This has also been reflected in the main text. Please see section IV-C and IV-D. } 

    \item \review{The left half of Fig.1 is a great overview but the right half is making the false promise that there is somehow a human in the loop.This figure needs to be revised to make clear that this is not an imitation learning method and doesn’t interact in any way with the human rollouts.} \\
    \answer{We have removed the right half of Fig.1. Please refer to the answer to meta-reviewer 1) for our changes related to human-likeness.}

    \item \review{Multimedia: Good, save for the things already addressed above (false positioning as human-like, etc)}\\
    \answer{We have toned down the human-likeness in the video as well as the main text. Please see the submitted revised movie.}

\end{enumerate}

\subsection{Reviewer6}
\begin{enumerate}
    \item \review{The main contribution is incremental, as both the parameter estimation and NMPC controller are re-implementations of CMA-ES and iLQR. The main contribution is the addition of the GP Regression on the system residuals, which uses a simple MLL and loss function.} \\ %\assign{MELCO-MERL} \\
    \answer{The proposed CMS system presents a complex non-linear dynamical system for real-time control. As we have pointed out in the related work section, previous work on using a full physics engine and a ML model for residual correction deals with rather simple dynamical systems~\cite{ajay2019combining}. Moreover, to the best of our knowledge, our work is the only work that makes use of a non-linear model predictive control (NMPC) policy in real-time when the underlying system is specified by a physics engine which is compensated for residuals using a ML model (as opposed to differential algebraic equations (DAEs) which requires domain knowledge to derive dynamics equations). Please note that this requires solution to continuous-time optimization problem in real-time where the gradients are computed using the physics engine and ML model. Most of the simplifications done (such as reducing the state-space of the physics engine) were done to make real-time computation feasible with available compute resources. Previous work using such a framework deals with quasi-static dynamics where MPC control problem was solved for discrete control inputs and thus was much simpler~\cite{ajay2019combining}. We have highlighted this at the end of section I and section II.
    }
    %As the reviewer accepts and described in Sec.~\ref{sec:intro}, the use of a hybrid model consisting of a full physics engine with a statistical function approximator is novel, and we would think this would be an enough contribution considering this method can be applied to arbitrary robotic tasks while it still needs some adaptation, such as system-level problems described in Sec.~\ref{sec:approach}.

    \item \review{There are several adaptations made to the general problem to get to the final experimental results - e.g. the simplification on the radius of each circle of the maze, the inverse modelling of motors, the reduction of the control problem to trajectory tracking. While each of these steps are logical and clearly explained, the overall result is much more ad-hoc to the task at hand and less general. In other words, the sim-to-real gap is being reduced by design, lessening the role of the residual learning}\\
    \answer{We thank the reviewer for raising this point. While we are aiming for generality, some domain knowledge is required for efficient performance in robotic systems or in any model-based controller implementation. We have highlighted our approximation and simplifications explicitly in Sections III and IV-B. As you can see, these simplifications are done to tackle actuation delays, the long horizon planning (in a task and motion planning setting) and discontinuities in the state-space of the system using some system-specific domain knowledge. However, those domain knowledge alone cannot solve the problem well. This can be concluded from our sim-to-sim and sim-to-real experiment. The sim-to-sim experiment in Fig. 3 shows that the default physics properties defined in a physics simulator cannot simulate well between the two simulators that have different dynamics. Without the parameter estimation step, the controller fails as it cannot overcome the static friction (and thus the marble does not move). With parameter estimation, the marble starts moving as the NMPC policy can compensate for some degree of uncertainty. With the additional GP correction, the marble movement becomes more precise and thus the marble can reach the goal faster.
    The sim-to-real experiment clearly shows that the proposed method improves the performance by comparing the results of "CMA-ES" and "CMA-ES + GP3" in Fig. 4.}
    
    %We would like to clarify the underlying motivation and thought process in making some simplifying assumptions for the proposed CMS. The proposed CMS is a complicated system for real-time control as the dynamics of the marble is affected by the geometry of the maze environment together with complex contact phenomena with the walls and friction. Apart from the complex dynamics, real-time control of the marble is difficult as the CMS is underactuated, and a policy has to plan for long planning horizon while accounting for several discontinuities. Furthermore, the CME is actuated by hobby-grade servo motors which suffer from significant delays (about $\sim 0.2$ seconds while the control loop runs at $30$ Hz, and thus the delay accounts for $6$ control steps).  In our case, we made some simplifications to the system dynamics to model the marble movement in polar coordinates (to allow real-time computation). The other simplification was to model the inverse motor model to model delay in actuation. }
    %Firstly, we would like to emphasize that the sim-to-real experiment is conducted on a relatively complicated system: the CMS includes constrained geometry, underactuated control, nonlinear dynamics, and a long planning horizon with several discontinuities. We would consider that it would be a common approach to use domain knowledge to solve such a complicated system in robot control.
    %In addition to this, you can see that only using those domain knowledge cannot solve the problem well from our sim-to-sim and sim-to-real experiment.
    %The sim-to-sim experiment in Fig.~\ref{fig:maze_with_traj_sim} shows that the default physics properties defined in a physics simulator cannot simulate well between the two simulators that have different dynamics. Also, the sim-to-real experiment clearly shows that the proposed method improves the performance by comparing the results of "CMA-ES" and "CMA-ES + GP3" in Figure~\ref{fig:comparison_CMAES_GP}.} % \assign{MELCO-MERL}

    \item \review{Another consideration is that of the experimental results. The comparison to human performance is made through an interface which is not usual for humans (the joystick controller and tilt-table). It is hard to establish a comparison of how much human experience with such system is equivalent to the sim-to-real parameter inference with collected environment observations. As such, it is not clear whether the performance gains are attributable to human unfamiliarity with such system or an overall better performance of the framework proposed.}\\
    \answer{As described in our response to the meta-reviewer 1), because people can adapt to joystick-based control quickly, and because do not find reliable performance gains, we believe that any improvements due to better familiarity would be slight at best.} % \assign{Kevin}

    % \item \review{Need of other baselines to compare how the method performs against other, preferably model-based, numerical methods}\\
    % \answer{We thank the reviewer for this question. In general, a NMPC control policy is robust to some degree of parametric uncertainty~\cite{findeisen2003state}. In our case, we found that using a NMPC policy without any learning was grossly inaccurate and was not able to move the marble due to static friction. We believe that the performance will be similar if one uses other non-linear programming based methods for MPC, and thus, we did not consider other similar approaches. The iLQR method used here was chosen for its compute advantages compared to other direct methods for trajectory optimization~\cite{tassa2012synthesis}.}  % \assign{MELCO-MERL}

    \item \review{Finally, meanwhile the method may have been inspired by the way humans learn or keep a physical model of the environment, the connection between the proposed framework and human behaviour is superficial, and therefore qualifications such as "human-like" may not be appropriate unless further subsidised.}\\
    \answer{We agree, and as mentioned in our response to the meta-reviewer's similar point, have changed the title, introduction, and discussion to reflect this.} % \assign{Kevin}

    \item \review{The last paragraph of section V.A could be clearer. Does it imply that the two set of parameters found show the same performance? Which was used eventually?}\\
    \answer{We apologize for the confusion. The two set of parameters shown in section V-A are for sim-to-sim and sim-to-real experiments, respectively. The computed physical properties for the sim-to-real experiment in section V-A are used for the experiments on section V-B. We have revised the section V-A and section V-B to clarify this.} % \assign{MELCO-MERL}
\end{enumerate}


\subsection{Reviewer7}
\begin{enumerate}
    \item \review{I’m curious how the SAC based approach works in the real world. The supplementary material seems to have results only for simulation and in most of the cases SAC has lower timings. If SAC performs so well then what’s the motivation for using a model-based method? I think it would be worth highlighting that as it leaves the reader confused.}\\
    \answer{Although the final performance of SAC in simulation is better than our method in terms of time to solve the task, it requires $\sim$1000 times more samples to train the policy compared to our method. Also, we have tried applying SAC to the real system, but it failed to train a meaningful policy within several days of training time. We clarify this in Supplementally Material.}

    \item \review{Did you use the GP uncertainty in trajectory optimisation?}\\
    \answer{In the current version of the paper, we do not use the uncertainty in trajectory optimization. Only the mean GP predictions are used during trajectory optimization. We have added this comment in section V-B for clarification.} 

    \item \review{Any generalisation experiments on different size of the marble?}\\
    \answer{This requires further exploration and has been left as a future exercise (as seen in the Conclusions section of the paper).}
\end{enumerate}


==> review.tex <==
\clearpage
\onecolumn


\newcommand{\emphasize}[1]{\textcolor{red}{\textbf{#1}}}

\section{Review}

\subsection{Meta-Review}
The reviewers agree that the paper is well-written and presents a sound method that combines a number of existing methods in a novel way. However, their following concerns should be addressed:

\begin{itemize}
    \item \emphasize{The motivation and positioning on being human-liked and human-level should be toned down. This includes the remarks in the video.}
    \item Although the authors provided a problem definition section with a list of limitations and assumptions, \emphasize{some important points raised by the reviewers (e.g. related to generality claim of the paper given it is verified in a single task, limitations related to GP, assumptions on distance metric) should be clearly listed/discussed.}
    \item A more detailed analysis could have been provided in the experimental validation.
    \item \emphasize{The contributions can be clearly stated at the end of the introduction}, clarifying the novelties with respect to the existing methods for each contribution.
\end{itemize}

Although I believe that such human experiments and comparisons are very valuable, \emphasize{I also believe that the experiments that compare the performance of the model with humans are not well-formed.} The
experimental design is not fully described as should be in human experiments (who are the subjects, are they naive to the task, do they have previous experience, etc.).
More importantly, I believe that \emphasize{the relatively poor performance of the humans might be due to the joystick based control of the platform (rather than physics predictions).
The video shows direct control of the platform; how is the performance of the humans in that condition?} The subjects are given one minute to play with the joystick and it was assumed that they learned inverse control model. How can the authors make sure that the control is learned in such short time? The authors can refer to the large body of motor control research (e.g. Amirshirzad et al. IEEE Transactions on Human-Machine Systems) for justification of the motor adaptation.

In the results section, "In the middle two rings, ... we can still observe an improvement in the reduction of the variability of the performance": this statement is not supported with data. Additionally, it is difficult to visually see the difference and even if there is slight difference, it is evident that such reduction is not significant. I suggest to remove that statement.

Two questions: 
\begin{itemize}
    \item  \emphasize{Why did the authors design a lower level controller to move the marble to the next ring? Does it not hurt the generality of the model statement? Did the authors try without such lower level controller?}
    \item \emphasize{It is not clear what is meant by 'the location of the marble is set to the center of each ring' considering that the forward model should "have the same state that can be observed in the real system"}
\end{itemize}

The authors are requested to address all the above and all reviewer comments in their revised version.

\subsection{Review2}
\paragraph{Summary}
The authors present a sim2real algorithm that trains an agent to solve a circular maze environment (CME) in simulation and transfers this through parameter estimation, an inverse model, and a residual model to a real robot.

\paragraph{Contributions}
Applying a selected range of existing methods (MPC, SystemID, augmented simulation) to a specific problem (CME). 

The paper presents a neat little application of a set of existing methods. The results are okay and the presentation adequate. 

That being said, the main problem is the motivation and positioning of the paper. \emphasize{This work vastly overstates its own importance and contribution and needs to be toned down before I can recommend submission.}
\emphasize{The paper claims that this method is general but provides no proof (even simulation-to-simulation), the paper sweeps under the rug the fact that many design decisions only work with this kind of problem (e.g. GP aren't feasible for higher-dimensional problems, the linear distance to nearest goal that's not feasible for concave paths/obstacles, the modeling of \_all\_ sim2real differences as a GP, including non-stationary effects), and the framing as "human-level" or "human-like" is slightly inappropriate.}
Maybe I missed something but the justification for that positioning was "Humans have an intuitive
physical understanding and they can learn dynamics on top of that and therefore we take an arbitrary simulator and an arbitrary machine learning model (Gaussian Process model)" (paraphrased from section 5.b).
In both the video and the paper, you mention multiple times this being inspired by cognitive science while giving no evidence that the actual underlying process in a human's mind is in any way comparable to what you're doing.
And more specifically, if you make vast claims like this, then I expect much more rigor in your experiments: Instead of just having a human baseline on a single task, I'd expect a behavior analysis of how quickly humans adapt to a variety of tasks (not just this one maze) and based on this, I'd expect you to pick from a range of machine learning methods that all serve the same purpose of fine-tuning the simulation.
\emphasize{What you presented in the current version of the paper has nothing to do with a "human-like" system other than using an augmented simulator} and if that's human-like, then dozens of works that have done the same thing over the last couple of years are also all human-like and therefore this is not a novel feature of your work.
If you could remove all references to human-likeness, your paper would be in a much better position. This includes the title which I'd reframe as something like "Solving a maze task via a learning-augmented simulator" (sidenote: the title also currently says "puzzles", plural, and I fail to see a plurality of puzzles).

Again, keep in mind that I find the core of the paper okay (i.e. the methods and results). I'm only recommending changing parts of the introduction, the start of the problem formulation section, and the conclusion. If you need to mention humans anywhere, then maybe point out that the performance of your model on this one specific task is better than human, but so are many ATARI RL agents, rock/paper/scissor robots, etc.

\subsubsection{Organization and Style}
\emphasize{I'd recommend the authors add a section to the end of the introduction summarizing their contribution in a bullet point or two and also stating clearly what is NOT in the scope of this work.}

\subsubsection{Technical Accuracy}
Mostly okay. \emphasize{The main results are presented only in a plot in Figure 4 and it's entirely unclear if the differences between models per ring are statistically significant. There is also no information on number of trials unless I missed something. Also the use of weight matrices is very unclear and feels important to the optimization processes (What is Q in eq.8? How did you arrive at 4,4,1,.4 for W in eq.6?)}

\subsubsection{Presentation}
\emphasize{The left half of Fig.1 is a great overview but the right half is making the false promise that there is somehow a human in the loop.} This figure needs to be revised to make clear that this is not an imitation learning method and doesn't interact in any way with the human rollouts. Fig.2 is great.

\subsubsection{Multimedia}
Good, \emphasize{save for the things already addressed above (false positioning as human-like, etc)}. Also, you misspelled Josh's last name.

\subsection{Review6}
The paper describes a framework based on non-linear model-predictive control (NMPC) to solve a marble-in-a-maze task. The approach combines an approximated physics engine model with a Gaussian Process (GP) to model the discrepancy between observed data and simulated data, i.e. the observed residuals.
The framework is applied to a real robotic system comprised of a circular maze environment controlled by a tip-tilt table (CMS) and compared against human performance baselines for the same task.

The submission is well written, with clear language, proper structure, and minimal typos. The main contribution claim is that the approach is inspired by the way humans learn and combines the sample efficiency of model based control with the flexibility of adjusting the model according to observations from the environment.
This in turn allows it to improve on human level performance while maintaining the same level of sample efficiency as well as learning a more useful model for sim-to-real applications. The amount of citations is adequate and the authors acknowledge on related work that the idea of residual modelling is not new and has been applied in several other instances, including a combination of MPC and residual modelling, albeit for a much simpler problem. Lastly, experimental section shows a comparison of the proposed method and humans interfacing with the CMS through a joystick, comparing the amount of time spent in each of the inner circles of the maze.

Although the results are encouraging and clearly show the effort spent on the implementation, there are a few issues that need to be addressed:
\begin{enumerate}
    \item \emphasize{The main contribution is incremental, as both the parameter estimation and NMPC controller are re-implementations of CMA-ES and iLQR. The main contribution is the addition of the GP Regression on the system residuals, which uses a simple MLL and loss function.} Notably, the fact that the framework relies on a possibly black-box physics engine is also novel, as is the real-time implementation. This undoubtedly required a lot of effort, but due to the several approximations may restrict the general applicability of the method, bringing to light the next point;
    \item \emphasize{There are several adaptations made to the general problem to get to the final experimental results - e.g. the simplification on the radius of each circle of the maze, the inverse modelling of motors, the reduction of the control problem to trajectory tracking.} While each of these steps are logical and clearly explained, the overall result is much more ad-hoc to the task at hand and less general. \emphasize{In other words, the sim-to-real gap is being reduced by design, lessening the role of the residual learning;}
    \item Another consideration is that of the experimental results. \emphasize{The comparison to human performance is made through an interface which is not usual for humans (the joystick controller and tilt-table).} It is hard to establish a comparison of how much human experience with such system is equivalent to the sim-to-real parameter inference with collected environment observations. \emphasize{As such, it is not clear whether the performance gains are attributable to human unfamiliarity with such system or an overall better performance of the framework proposed.} Understandably, the paper might want to keep such distinction unclear, as the compounded result might be the final goal, however it still brings to light the need of other baselines to compare how the method performs against other, preferably model-based, \_numerical\_ methods.
    \item Finally, meanwhile the method may have been inspired by the way humans learn or keep a physical model of the environment, \emphasize{the connection between the proposed framework and human behaviour is superficial, and therefore qualifications such as "human-like" may not be appropriate unless further subsidised.}
\end{enumerate}

Minor suggestions:
\begin{itemize}
    \item In section IV.B there is a typo: psuedo instead of pseudo
    \item \emphasize{The last paragraph of section V.A could be clearer. Does it imply that the two set of parameters found show the same performance? Which was used eventually?}
    \item A contemporaneous work which could be added to related work is [1], which addresses using black-box physical engines with model-free and model-based control.\\
    R. Possas, L. Barcelos, R. Oliveira, D. Fox, and F. Ramos, Online Bayes Sim for Combined Simulator Parameter Inference and Policy Improvement, International Conference on Intelligent Robots and Systems (IROS), 2020, p. 8.
\end{itemize}

\subsection{Review7}
The paper proposes a method to learn to solve puzzles (circular maze environment where the task is to get the marble to the center of the maze) using a combination of simulated and the real world data.
They create a simulated environment of the same scene and first calibrate the physics parameters by collecting real world data and using CMA-ES. Next, they model the residual (difference in the dynamics model of simulated and real world scene) function with a Gaussian Process. Last they use this learned model to optimise the trajectory of the marble using iLQR.

I'm curious how the SAC based approach works in the real world. The supplementary material seems to have results only for simulation and in most of the cases SAC has lower timings. If SAC performs so well then what's the motivation for using a model-based method? I think it would be worth highlighting that as it leaves the reader confused.
Overall, I liked the work and the attention to details e.g. learning inverse model for action delays, modelling the residuals after calibration etc. and using a model based method. I think the choice of
the environment is also great.
Few questions- 
\begin{itemize}
    \item Did you use the GP uncertainty in trajectory optimisation?
    \item Why no experiments with model-free RL methods in the real world?
    \item Any generalisation experiments on different size of the marble?
\end{itemize}
